Computational Tradeoff in Minimum Obstacle Displacement Planning for Robot Navigation

In this paper, we look into the minimum obstacle displacement (MOD) planning problem from a mobile robot motion planning perspective. This problem finds an optimal path to goal by displacing movable obstacles when no path exists due to collision with obstacles. However this problem is computationally expensive and grows exponentially in the size of number of movable obstacles. This work looks into approximate solutions that are computationally less intensive and differ from the optimal solution by a factor of the optimal cost.

==> optimization_problem.tex <==
The optimization problem that we will state in the following has the objective to determine the best trajectory for the robot to reach the desired position by limiting the displacement of the obstacles during the robot's motion. Constraints to be included are the collision avoidance between the robot and the obstacles and upper lower bounds for state and control variables.
The overall optimization problem is formalized as:
 \begin{equation}
     {\text{min}} \quad J^{R}+J^{O}  \label{obj_tot}
 \end{equation}
\begin{equation}
    J^{R}= \sum_{k\in K} \left ( r^{x}_{k}-r^*_{x}\right )^2+\left ( r^{y}_{k}-r^*_{y}\right )^2
\end{equation}
\begin{equation}
    J^{O}= \sum_{k\in K}\sum_{o\in \mathcal{O}} \left ( d^{x}_{o,k}\right )^2+\left ( d^{y}_{o,k}\right )^2 
\end{equation}
\begin{equation}
     r^{x}_{k+1}= r^{x}_{k}+\tau v^{x}_{k}+\frac{\tau^2}{2} a^{x}_{k} \quad k \in {K} \label{x_r1}
\end{equation}
\begin{equation}
     r^{y}_{k+1}= r^{y}_{k}+\tau v^{y}_{k}+\frac{\tau^2}{2} a^{y}_{k} \quad k \in {K} \label{y_r1}
\end{equation}
\begin{equation}
    v^{x}_{k+1}=v^{x}_{k}+\tau a^{x}_{k} \quad k \in {K} \label{v_x1}
\end{equation}
\begin{equation}
    v^{y}_{k+1}=v^{y}_{k}+\tau a^{y}_{k} \quad k \in {K} \label{v_y1}
\end{equation}
\begin{equation}
    |\left (r^{x}_{k}-x_{o,k}\right )+\left (r^{y}_{k}-y_{o,k}\right )| \geq R_r+R_o \quad o \in \mathcal{O} \quad k \in {K}
    \label{eq:coll_con}
\end{equation}
\begin{equation}
    \underline{x} \le x_{k}\le \overline{x}  \quad k \in {K}
\end{equation}
\begin{equation}
    \underline{u} \le u_{k}\le \overline{u}  \quad k \in {K}
\end{equation}
\begin{equation}
    \underline{x^O} \le x_{o,k}\le \overline{x^O} \quad o \in \mathcal{O} \quad k \in {K}
\end{equation}\begin{equation}
    \underline{y^O} \le y_{o,k}\le \overline{y^O} \quad o \in \mathcal{O} \quad k \in {K}
\end{equation}
\begin{equation}
    \underline{d^x} \le d^x_{o,k}\le \overline{d^x} \quad o \in \mathcal{O} \quad k \in {K}
\end{equation}
\begin{equation}
    \underline{d^y} \le d^y_{o,k}\le \overline{d^y} \quad o \in \mathcal{O} \quad k \in {K}
    \label{eq:d_y}
\end{equation}
Problem \eqref{obj_tot}-\eqref{eq:d_y} is a nonlinear and nonconvex problem due to the collision avoidance constraint \eqref{eq:coll_con}. The previous condition can be linearized through the introduction of binary auxiliary variables $\xi^1_{o,k}, \xi^2_{o,k}, \xi^3_{o,k}, \xi^4_{o,k} \in \left \{0,1\right \}$ as follows:
\begin{equation}
    r^{x}_{k}-x_{o,k} \geq R_r+R_o-\xi^1_{o,k}M \quad o \in \mathcal{O} \quad k \in {K}
\end{equation}
\begin{equation}
    -\left(r^{x}_{k}-x_{o,k}\right) \geq R_r+R_o-\xi^2_{o,k}M \quad o \in \mathcal{O} \quad k \in {K}
\end{equation}
\begin{equation}
    r^{y}_{k}-y_{o,k} \geq R_r+R_o-\xi^3_{o,k}M \quad o \in \mathcal{O} \quad k \in {K}
\end{equation}
\begin{equation}
    -\left(r^{y}_{k}-y_{o,k}\right) \geq R_r+R_o-\xi^4_{o,k}M \quad o \in \mathcal{O} \quad k \in {K}
\end{equation}
\begin{equation}
    \xi^1_{o,k}+\xi^2_{o,k}+\xi^3_{o,k}+\xi^4_{o,k} \leq 3 \quad o \in \mathcal{O} \quad k \in {K} \label{lin_end}
\end{equation}
where $M$ is an appropriate large constant. Thanks to this formulation the problem now is e Mixed Integer Quadratic Program (MIQP).
